Deep Unlearning via Randomized Conditionally Independent Hessians

Recent legislation has led to interest in machine unlearning, i.e., removing specific training samples from a predictive model as if they never existed in the training dataset. Unlearning may also be required due to corrupted/adversarial data or simply a user's updated privacy requirement. For models which require no training (k-NN), simply deleting the closest original sample can be effective. But this idea is inapplicable to models which learn richer representations. Recent ideas leveraging optimization-based updates scale poorly with the model dimension d, due to inverting the Hessian of the loss function. We use a variant of a new conditional independence coefficient, L-CODEC, to identify a subset of the model parameters with the most semantic overlap on an individual sample level. Our approach completely avoids the need to invert a (possibly) huge matrix. By utilizing a Markov blanket selection, we premise that L-CODEC is also suitable for deep unlearning, as well as other applications in vision. Compared to alternatives, L-CODEC makes approximate unlearning possible in settings that would otherwise be infeasible, including vision models used for face recognition, person re-identification and NLP models that may require unlearning samples identified for exclusion. Code can be found at https://github.com/vsingh-group/LCODEC-deep-unlearning/

==> inputs/_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}


==> inputs/_discussion.tex <==
\section{Discussion and Broader Impacts}
\ronak{should this be intro or discussion?}
With personal data becoming one of the most valuable commodities, legislative effort has begun to push back on widespread and unilateral collection.
Particular focus has been put towards the ``right to be forgotten" (RTBF), establishing the right of an individual's data to be deleted such that no other party may access it.
Even among existing legal frameworks on copyright and fair use, industry scraping has led to large numbers of personal images being used without proper consent from subjects \cite{Exposing}.
Large amounts of this data collection are not only stored for descriptive statistics, but now commonly used in training complex models.
While recent regulation (GDPR, CCPA) has not always specified the extent to which data must be forgotten, this poses a clear question: is simple deletion of the original data enough, or does any model built on that data need to be updated as well?

Recent work has identified situations in which trained models are vulnerable to attacks that can reconstruct input training data \cite{carlini2019secret,carlini2020attack}. More directly, a recent ruling by the Federal Trade Commission ordered a California company to delete any model or algorithm ``using the photos and videos uploaded by its users" \cite{ftc}.
While full model deletion and retraining without the users' data is possible, many models deployed require several weeks of training, with up to millions of dollars in computational resource allocation. With additional deletions, it is infeasible to retrain each time a request to delete is made. This begs the question: Are there updates to the model that ensure the data has been deleted, but do not require full retraining?
Existing work has answered this in the affirmative as noted above, computational burden has limited their more broad use and application.
% . Recent results under a theoretical framework of forgetting have established models and criteria that provide updates to models with guarantees that data has been effectively removed. Many of these updates require full computations of the Hessian at the point of removal, which is infeasible in large neural networks typically used in the industry for high-dimensional vision recognition tasks.

Here we provide a more efficient procedure, taking advantage of a block-coordinate update informed by conditional independence. Using a simple adaptation of a new measure for CI, we are able to effectively identify the most important set of parameters to update, to ensure a sample's influence is properly scrubbed from a model.
Future work could involve a complete evaluation of our method in specific, real-world applications such as person-identification. There is room for interesting theoretical insights as well, with potentially strong connections to both differential privacy and sample influence.

==> inputs/_sample.tex <==
{\bf Functional Leverage Score Estimation for Sublinear Unlearning.}
\sathya{Use leverage scores instead of Fischer information matrix to motivate this section. }
While the above assumes a sample to be scrubbed is provided, in other situations a user may require a set of samples $T$ to be unlearned. In this case the above procedure needs to be run over all elements in the set. 
However, we can take advantage of linearized approximations to enable yet another one-shot procedure.
%given that our approach is explicitly evaluating where in the parameter space a sample needs to update, 
%we can apply this approach to selecting samples to unlearn through their overall \textit{influence}.
%If only a subset of samples have a high influence, it may only be necessary to unlearn a smaller set $<<|T|$.
Under some assumptions, we can describe the parameters of a model as a linear combination of the input data,
\begin{align}
    w(s) = \sum_{i=1}^{|S|} s_i f(z_i, w)
\end{align}
Using a linearization about the point where $s_i = 1 \forall i$, we can estimate the parameters where $s_i = 0$ for some samples, as in \cite{koh2017understanding},
\begin{align}
    \bar{w} = \hat{w} - [\nabla^2 F(\hat{w})]^{-1|}] \nabla F_T (\hat{w}) 
\end{align}
This result can be applied directly to a set of candidate deletions $T$: if we know the influence of a set of samples in $T$ is low (where $s_i=0$, then we can ignore them in our update procedure. Using other existing methods that take advantage of this linearization to estimate influence \cite{harutyunyan2021estimating}, we can select the samples in $T$ that have a large influence and remove them.
Using a linearized version to compute an approximate function sample (mutual) information as 
\begin{align}
    F-SI \approx \frac{1}{2\sigma^2 n_{val}} (w - w_{\setminus i})^T (H_{val} - \lambda I) (w - w_{\setminus i})
\end{align}
Practically, $H$ is difficult to compute even under the linearized setting, and their final score ends up being a simple squared difference between the parameters before and after the rank-1 update to get $w_{\setminus i}$.
Instead, we can again instantiate the correlation version of L-CODEC, and compute a sample influence measure as $T(w, w_{\setminus i})$, where the individual parameters serve as samples for the random variable representing the network state with and without that sample.

% don't have to unlearn all samples given to unlearn?
% use sample influence to choose samples to remove

% under linearized, we can compute this 

% %{\color{red} TODO dual formulation of unlearning...}

% (1-codec) for ``informativeness"

% For any problem in which we may want to estimate the impact of a sample on a networks' output, we often approximate via a second order estimation:
% \begin{align}
% d(s) :&= \EE_x[||f_w(x) - f_{w_{\setminus s}}(x)||^2] \\
% &\approx (w - w_{\setminus s})^\top \Sigma^{-1}_w (w - w_{\setminus s})
% \end{align}
% where $\Sigma^{-1}$ is approximated via a Hessian or Fisher matrix.


% \begin{outline}[enumerate]
% \1 traditional setups
%     \2 formalize, difference in model output with and without sample
%     \2 conditional mutual information setup: 
%     $w \bot s_i | s_{\setminus i}$
% \1 strict def requires 
%     \2 distributional estimation
%     \2 using upper bound estimate of marginals
% \1 common to add noise to get distributional, seeds are not sufficient
%     \2 assume gaussian, get nice dists.
% \1 instead, we can consider each weight parameter as an example of the networks' output
%     \2 and compute the correlation between weights with and without
% \end{outline}

% \begin{align}
%     f_\theta &\bot s_i | s_{\setminus i} \\
%     f_\theta &\bot s_i | s_{\setminus i}
% \end{align}

% \subsubsection{Linearizations}
% \begin{outline}[enumerate]
% \1 effect of sample on weights would require retraining in full
%     \2 not feasible...
% \1 NTK linear approximation
%     \2 2 sentence overview
%     \2 definition a la soatto
% \1 weights here are directly computed by ntk
% \end{outline}

==> inputs/_sever.tex <==
\subsection{Approximately Robust Model Selection with SEVER}

Direct application of SEVER does not work in the case when the size of the model $w$ is large. In this case it is not possible to compute the full singular value decomposition of $G$. Instead, we can compute the thin-SVD.


Even though we cannot guarantee the smallness of the subset identified by FOCI, in practice it has been observed, and we observe, that selected sets are quite small ($\approx O(log(d)$). 


\begin{algorithm}
\SetAlgoLined
\KwData{trained model $\hat{w}$, training set used for model $X$, filtering threshold parameter $\sigma$}
\KwResult{Robust model $\hat{w}$}
Inlier set $S = \{1,\ldots,|X|\}$ \\
 \While{stopping condition}{
  Compute gradients $\nabla f(\hat{w}, x_i)\ \forall i \in S$. \\
  Compute $\hat{\nabla} = \frac{1}{|S|}\sum \nabla f(\hat{w}, x_i)$. \\
  
  $G = [\nabla f(\hat{w},x_i) - \hat{\nabla}]_i$. \tcp*[f]{Compute centered gradients}\\
  Compute the thin SVD of $G$, and the top right singular vector as $v$. \\
  
  $\tau_i = \left((\nabla f(\hat{w},x_i) - \hat{\nabla})\dot v\right)^2$. \tcp*[f]{Compute outlier scores}\\
  
   $T^\prime = FILTER(S, \tau, \sigma)$. \tcp*[f]{Identify outliers via filtering} \\
  
  $\hat{w} = FOCISCRUB(\hat{w}, T^\prime)$. \tcp*[f]{unlearn outliers}\\
  $S = S \setminus T^\prime$. 
 }
Return robust $\hat{w}$, inlier set $S$.
 \caption{Unlearning with Outlier Filtering}
\end{algorithm}

\begin{algorithm}
\SetAlgoLined
\KwData{scores $\tau_i$, filtering threshold parameter $\sigma$.}
\KwResult{Outlier set $T$}
   $T^\prime = FILTER(S, \tau, \sigma)$. \tcp*[f]{Identify outliers via filtering} \\
Return outlier set $T^\prime$.
 \caption{Outlier Selection}
\end{algorithm}

\begin{algorithm}
\SetAlgoLined
\KwData{trained model $\hat{w}$, samples to unlearn $x_i$, $i \in T$}

For each sample $i$ \\
Run a forward pass for $x_i$ \\
Construct hypercolumn. \\
Run FOCI on vectorized hypercolumn, \\ identifying a minimal subset that makes the rest conditionally independent of the input. \\
Run the unlearning step described in (X), where the parameters updated and the hessians computed are only those of the filters associated with the FOCI selected hypercolumns.
\caption{FOCI Unlearning}
\end{algorithm}

Thin SVD is still not good enough for datasets sizes of 10K+.

With this, we need a way of reducing the dimensionality of $G$.

\begin{enumerate}
    \item Median image through network, FOCI hypercolumn select.
\end{enumerate}


==> inputs/_spectra.tex <==

\ronak{maybe leave this out?}
\subsection{On the Conditioning of the Hessian}
\begin{proposition}
Let $X \in \RR^d$ and $Y \in \RR$ be random variables. The feature subset selected by FOCI(X,Y), $s \subseteq [d]$ are also conditionally linearly independent.
\end{proposition}
\begin{proof}
If there does not exist any measure function between $Y$ and $X\setminus Z$ given $Z$, then clearly there also does not exist any linear function.
%Global conditional independence implies conditional linear independence, and linear dependence generally cannot be changed by a linear condition. In other words, 
%Suppose there is some set $Z \subset X$ such that $Y$ is linearly independent of $X\setminus Z$ given $Z$. Then there exists no function $f(Y,Z)$ such that 
%\begin{align}
%f(Y,Z) = \sum_{i\in [|X\setminus Z|\} a_i X_i
%\end{align}
%for nonzero $a_i$.

%If there do not exist nonzero coefficients $a_i$ such that $Y = \sum a_i X_i$ ($Y$ linearly independent of  $X$), then no subset of  
%Conditional linear independence for a subset of features $Z$ that there are no such coefficients 
%$Y = \sum_{i=1}^d a_i X$
%Conditional linear independence:
%X indep Y | Z =>
%there are no coeffs such that ax + by 
%Let $X \in \RR^{n \times d}$ be a sample of $d$ features with size $n$. 
%FOCI chooses elements to add to the sufficient set that maximally reduce any measurable dependence between those left over and the output $Y$. 
\end{proof}
\begin{proposition}
The condition number of the covariance matrix computed over the FOCI-selected ordering of features is monotonically increasing (generally).
\end{proposition}
If features are selected to be added to the subset, then they must have some measurable effect on our understanding of $Y$. Each additional feature selected must also increase our understanding of $Y$. If there were a strong linear dependence among features $Z_i$ and $Z_j$ in the selected set, then the collective effect on $Y$ could be written as $a Z_i + b Z_j$ for some nonzero $a,b$. Because FOCI selection is not dependent on linearity, the measurable effect on $Y$ must be equal or similar. In this case, only one of the two features would be chosen, and others in the set would have to contribute to $Y$ through an independent path.

This result first seems counterintuitive; large condition numbers at optimality are bad. However, if our goal is to remove as much information related to a specific input as possible, it is \textit{in our interest} to identify the parameters with the largest impact. If FOCI is identifying parameters in order of their eigenvalue, then we know that each additional element added to the conditioning set can only decrease the minimum eigenvalue.
This has an additional benefit of keeping the condition number small and making the matrix inverse computation more ``nice".

Using these results, we can see that the unlearning algorithm \ref{alg:blockunlearn} is well-behaved. The quality of the inverse Hessian estimation is by definition controlled by the matrix condition number, and as such selecting only the subset of parameters that are linearly independent lead to parameter updates that will not be problematic due to practical problems with highly dependent features. Additionally, the selected descent directions will naturally be orthogonal, ensuring that even though a smaller subset of parameters are updated, those parameters represent diverse and complete information with respect to the sample of interest. 

==> inputs/_theory_old.tex <==


\subsection{Analysis}

We make use of the following observation made by many \cite{???}: models trained on complex tasks tend to \textit{delegate} subnetworks to specific regions of the input space. Example: The activation maps for different filters in a trained (converged) CNN model show differences for different classes specifically deeper in the network. 

Based on the above observations we make the following assumption:

\begin{assumption}
\begin{align}
    \forall S \sim \mathcal{P}(\mathcal{X}, \mathcal{Y}) \quad \exists T \subset L \\
    s.t., \quad \mathcal{L}(S) \bot w^{*}_{L\setminus T} | w^{*}_T
\end{align}
\end{assumption}
where, $S$ is the set of data points sampled from the joint training distribution of $\mathcal{P}(\mathcal{X}, \mathcal{Y})$, $w^*$ are the model parameters for a trained converged model, $L$ is the set of all layers (filters), $T$ is the subset of all layers which we will later tie to our selection algorithm. $\mathcal{L}$ is the loss function. 
Note: $S$ can be a singleton containing only one data point to be removed. It is most beneficial to think of $S$ as a set of data points belonging to a particular class. 

Input perturbation to get samples for FOCI computation: Given a data point $(x_k, y_k)$ from the training set $D$ we want to remove it. So, we perturb the input by adding small amount of Gaussian noise to generate samples for it. We have,

\begin{align}
    (x_k, y_k) \in D \xrightarrow[\text{perturbation}]{\text{input}} \{(x_k +g_k, y_k) | g_k \sim \mathcal{N}(0,1)\} = S_k
\end{align}
So, $S_k$ becomes our set S in \textbf{Assumption 1}. We generate sample for FOCI of the form $(\mathcal{L}(S_{k_i}), w^*(S_{k_i}))$; where $S_{k_i}$ is the $i$th perturbation of $x_k$ from set $S_k$ and $\mathcal{L}(S_{k_i})$ is the loss for the corresponding perturbation. 
After this $FOCI({(\mathcal{L}(S_{k_i}), w^*(S_{k_i})) | S_{k_i} \in S_k})$ gives us the required $T \subset L$ selection; i.e. selects $T$ out of $L$ layers in the model following \textbf{Assumption 1}. 

Now, we derive a bound on the residual gradient norm after removal. Residual gradient is defined as the gradient for the data points that are not being removed. Let us take $D$ to be the training set; w.l.o.g. $(x_k, y_k)$ is the point being removed. We have residual data $D' = D - {(x_k, y_k)}$.

Let use denote $w^-_{Full}$ as the weight parameters after doing a full Hessian update and $w^-_{Foci}$ as the weight parameters after doing a FOCI selected Hessian update. In an ideal case, we want $(w^-_{Foci}, D')$/$(w^-_{Full}, D')$ to be as close as possible to $(w^*, D')$. Note that we consider both $(w^*, D)$ and $(w^*, D')$ to be $0$ as we don't expect model parameters to change drastically for one sample once trained to convergence. 

Next, we define the residual gradient norm. Considering simplistic case for now, we think of $w$ to be a network of many linear layers with possible activation functions; we can think of the above norm as the sum of norm of gradients for each layer. Hence, for any model parameters $w$ and dataset $D$, we have:
% strong assumption here, tbd add details

\begin{align}
    \label{eq:res_norm}
    ||\nabla \mathcal{L}(w,D)||_2 \coloneqq \sum_{l \in L} ||\nabla \mathcal{L}(w_l, D) ||_2
\end{align}

As mentioned before, we have this selection from FOCI which based on what sample to remove gives us a subset $T$ of $L$ (set of all layers in the model). Let $R = L \setminus T$. So, $R$ is the remainder of the network which is not updated when doing a FOCI selected updated. Hence, \ref{eq:res_norm} for $(w^-_{Foci}, D')$ can be written as:

\begin{align}
    \label{eq:foci_res_norm}
    ||\nabla \mathcal{L}(w^-_{Foci},D')||_2 \coloneqq \sum_{l \in L} ||\nabla \mathcal{L}(w^-_{Foci_l}, D') ||_2 \\
    = \sum_{l \in T} ||\nabla \mathcal{L}(w^-_{Foci_l}, D') ||_2 + \sum_{l \in R} ||\nabla \mathcal{L}(w^-_{Foci_l}, D') ||_2 \\
    = \sum_{l \in T} ||\nabla \mathcal{L}(w^-_{Foci_l}, D') ||_2 + \sum_{l \in R} ||\nabla \mathcal{L}(w^*_{l}, D') ||_2
\end{align}
The last line follows from the fact for layers in $R$, they are not updated.

Now, although for certain layers weights haven't been updated, but the inputs to these layers may change due to updates in the lower layers. We will next show how for the remainder of the dataset $D'$ these changes propagate minimally when there are a large number of data points, $n$ in the training set.

W.L.O.G. assume that we have a $4$ layer network and the output is seen as:
\begin{align}
    L_4(L_3(L_2(L_1(x))))
\end{align}
For the point being removed $x \in D$; let $L_2$ be the intermediate layer which is selected for update by FOCI. Note: $a$'s below refer to activation form respective layers. 

Before update, activations out of $L_2$:
\begin{align}
    a_2 = L_2(L_1(x)) = L_2(a_1)
\end{align}
After update, activations out of $L_2$:
\begin{align}
    a_2' & = L_2'(L_1(x)) \\
    & = L_2'(a_1) \\
    & = w_2' \times a_1 \\
    & = (w_2 + \delta_{w_2}) \times a_1 \\
    & = w_2 \times a_1 + \delta_{w_2} \times a_1 \\
    & = a_2 + \delta_{w_2} \times a_1
\end{align}
Second line follows since $L_1$ isn't updated. Also, we have considered simple linear layers now. 

Let's next see how these effect activations out of $L_3$
Before, update:
\begin{align}
    a_3 = L_3(a_2)
\end{align}
After update:
\begin{align}
    a_3' &= L_3(a_2') \\
    &= L_3(a_2 + \delta_{w_2} \times a_1) \\
    &= L_3(a_2) + \nabla L_3 (a_2) \delta_w_2 \times a_1 + \mathcal{O}((\delta_{w_2} \times a_1)^2) \\
    &= L_3(a_2) + 0 + \mathcal{O}((\delta_{w_2} \times a_1)^2) 
\end{align}
Note, $L_3$ wasn't selected for update. Since, $L_3$ wasn't updated activations remain same as before and we have already assumed that model was trained to convergence, so the second terms is zeroed out. 

Now, we look at what $\delta_{w_2}$ looks like for the \cite{sekhari2021remember} update.
\begin{align}
    \delta_{w_2} = \frac{1}{(n-1)}(\hat{H}^{-1})\sum_{z \in \{(x_k, y_k)\}} \nabla f(\hat{w}, z)
\end{align}
Hence, $\delta_{w_2}^2 \propto \frac{1}{n^2}$. Therefore, for large values of $n$, the third term in the equation above approaches $0$. So, $a_3' = L_3(a_2)$. This shows that propagation is minimal. Similar arguments regarding null space for over-parameterized deep networks have been mentioned in \cite{golatkar2020forgetting}. 

Now, looking back at the residual gradient norm, we have:
\begin{align}
    \label{eq:foci_res_norm_simplified}
    ||\nabla \mathcal{L}(w^-_{Foci},D')||_2 = \sum_{l \in T} ||\nabla \mathcal{L}(w^-_{Foci_l}, D') ||_2 + \\
    \sum_{l \in R} ||\nabla \mathcal{L}(w^*_{l}, D') ||_2
\end{align}
Based on the above argument of minimal propagation, the second term above is $0$ as for layers in $R$, the weights haven't changed as well.
Therefore,
\begin{align}
    \label{eq:foci_res}
    ||\nabla \mathcal{L}(w^-_{Foci},D')||_2 = \sum_{l \in T} ||\nabla \mathcal{L}(w^-_{l}, D') ||_2 
\end{align}
and 
\begin{align}
    \label{eq:full_res}
    ||\nabla \mathcal{L}(w^-_{Full},D')||_2 = \sum_{l \in L} ||\nabla \mathcal{L}(w^-_{l}, D') ||_2 
\end{align}
Since, FOCI selects sufficient sets, we have $T \subset L$. Hence, 
\begin{align}
    ||\nabla \mathcal{L}(w^-_{Foci},D')||_2 < ||\nabla \mathcal{L}(w^-_{Full},D')||_2 
\end{align}
Therefore, the residual gradient norm is bounded lower for Foci selective update as compared to a Full update, for the same update rules. 




% For the samples in the training set:
% \begin{assumption}
% For all subsets of samples $S \subset D$, there exists a subset of the model parameters $P \subset \Theta$ such that 
% \begin{align}
%     L(S) \bot w_{\Theta\setminus P}^* | w_{P}^*
% \end{align}
% \end{assumption}



% \begin{theorem}
% The change in the activation of a layer $l_{i+1}$ after an update to a previous one is bounded as:
% \begin{align}
%     |l_{i+1}(\tilde{a}_i) - l_{i+1}(a_i)| \leq \frac{2ML^2m^2}{\lambda^3 n^2}
% \end{align}
% \end{theorem}
% \begin{proof}
% Let the output of the previous layer be given as $w_l * a_{l-1}$, and the scrubbed output be $\tilde{w}_l * a_{l-1}$. Then we can Taylor expand around the output of the next layer for the previous  $l_{i+1}(\tilde{w}_l a_{l-1})$:
% \begin{align}
%     l_{i+1}(\tilde{w}_l a_{l-1}) &= l_{i+1}((w_l + \Delta) a_{l-1}) \\
%     &= l_{i+1}(w_l a_{l-1}) + \nabla l_{i+1}(w_l a_{l-1}) \Delta + O(\Delta^2)
% \end{align}
% where $\Delta = \tilde{w}_l - w^*_l$, or the Sekhari update:
% \begin{align}
%     \Delta = \frac{1}{n+1}H^{-1} \nabla f(x_r).
% \end{align}
% The first-order term vanishes, because the gradient at the original point $w_l$ is 0 given that we've trained

% %For a specific parameter layer, the linear assumption allows us to use a form of convexity (?). 
% From Lemma 6 in Appendix C.1 of  \cite{sekhari2021remember}, we have that 
% \begin{align}
%     |w^* - \tilde{w}| \leq \frac{2mL}{\lambda n},
% \end{align}
% so 
% \end{proof}

% \begin{theorem}
% Residual Gradient norm
% \end{theorem}
% \begin{proof}

% \end{proof}

